Multi-Agent Reinforcement Learning Based on Representational Communication for Large-Scale Traffic Signal Control

Traffic signal control (TSC) is a challenging problem within intelligent transportation systems and has been tackled using multi-agent reinforcement learning (MARL). While centralized approaches are often infeasible for large-scale TSC problems, decentralized approaches provide scalability but introduce new challenges, such as partial observability. Communication plays a critical role in decentralized MARL, as agents must learn to exchange information using messages to better understand the system and achieve effective coordination. Deep MARL has been used to enable inter-agent communication by learning communication protocols in a differentiable manner. However, many deep MARL communication frameworks proposed for TSC allow agents to communicate with all other agents at all times, which can add to the existing noise in the system and degrade overall performance. In this study, we propose a communication-based MARL framework for large-scale TSC. Our framework allows each agent to learn a communication policy that dictates "which" part of the message is sent "to whom". In essence, our framework enables agents to selectively choose the recipients of their messages and exchange variable length messages with them. This results in a decentralized and flexible communication mechanism in which agents can effectively use the communication channel only when necessary. We designed two networks, a synthetic $4 \times 4$ grid network and a real-world network based on the Pasubio neighborhood in Bologna. Our framework achieved the lowest network congestion compared to related methods, with agents utilizing $\sim 47-65 \%$ of the communication channel. Ablation studies further demonstrated the effectiveness of the communication policies learned within our framework.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

In this paper, we propose a novel communication mechanism in which agents are effectively able to learn (i) \textit{which part of the message} is worth sending (ii) \textit{when} to send a message, and (iii) \textit{to whom} should the message be sent. This becomes useful, especially, in problems where there exist constraints on communication, for instance, limited bandwidth. Further, our proposed framework is differentiable which allows for end-to-end training.

We test our framework, QRC-TSC, on a real-world problem of traffic signal control, where the goal is to select the phases of the traffic signals and reduce congestion throughout the network. We also compare QRC-TSC to the state-of-the-art frameworks involving communication and show that QRC-TSC outperforms all of them by learning optimal communication protocols. We further perform ablation studies to investigate both the content of the messages learned within our framework and the effectiveness of communication policies. Further, QRC-TSC is a generic framework, which can be applied to various multi-agent problems.

Some real-world problems do have constraints like a cost of communication. Although we do not conduct a study on such a problem, we believe that QRC-TSC can be extended to include such a cost. One of the drawbacks QRC-TSC is that the maximum length of the message needs to be set apriori. One solution to this problem would be to allow multiple communication passes. We leave this for future work.




